ECCE unpolarized TMD measurements

We performed feasibility studies for various measurements that are related to unpolarized TMD distribution and fragmentation functions. The processes studied include semi-inclusive Deep inelastic scattering (SIDIS) where single hadrons (pions and kaons) were detected in addition to the scattered DIS lepton. The single hadron cross sections and multiplicities were extracted as a function of the DIS variables $x$ and $Q^2$, as well as the semi-inclusive variables $z$, which corresponds to the momentum fraction the detected hadron carries relative to the struck parton and $P_T$, which corresponds to the transverse momentum of the detected hadron relative to the virtual photon. The expected statistical precision of such measurements is extrapolated to accumulated luminosities of 10 fb$^{-1}$ and potential systematic uncertainties are approximated given the deviations between true and reconstructed yields.

==> acknowledgements.tex <==
\section{Acknowledgements}
\label{acknowledgements}

We thank the EIC Silicon Consortium for cost estimate methodologies concerning silicon tracking systems, technical discussions, and comments.  We acknowledge the important prior work of projects eRD16, eRD18, and eRD25 concerning research and development of MAPS silicon tracking technologies.

We thank (list of individuals who are not coauthors) for their useful discussions, advice, and comments.

We acknowledge support from the Office of Nuclear Physics in the Office of Science in the Department of Energy, the National Science Foundation, and the Los Alamos National Laboratory Laboratory Directed Research and Development (LDRD) 20200022DR.


==> author_list.tex <==
\affiliation{\AANL{2}}
\affiliation{\AcademiaSinica{2}}
\affiliation{\AUGIE{2}}
\affiliation{\BGU{2}}
\affiliation{\BNL{2}}
\affiliation{\BrunelUniversity{2}}
\affiliation{\CanisiusCollege{2}}
\affiliation{\CCNU{2}}
\affiliation{\Charles{2}}
\affiliation{\CIAE{2}}
\affiliation{\CNU{2}}
\affiliation{\Columbia{2}}
\affiliation{\CUA{2}}
\affiliation{\CzechTechUniv{2}}
\affiliation{\Duquesne{2}}
\affiliation{\Duke{2}}
\affiliation{\FIU{2}}
\affiliation{\GeorgiaState{2}}
\affiliation{\Glasgow{2}}
\affiliation{\GSI{2}}
\affiliation{\GWU{2}}
\affiliation{\Hampton{2}}
\affiliation{\HEAROKEK{2}}
\affiliation{\HUJI{2}}
\affiliation{\IJCLabOrsay{2}}
\affiliation{\IMP{2}}
\affiliation{\Inha{2}}
\affiliation{\IowaState{2}}
\affiliation{\IPAS{2}}
\affiliation{\JAEA{2}}
\affiliation{\JazanUniversity{2}}
\affiliation{\JeonbukNational{2}}
\affiliation{\JLab{2}}
\affiliation{\JMU{2}}
\affiliation{\KobeUniversity{2}}
\affiliation{\KoreaUniversity{2}}
\affiliation{\Kyungpook{2}}
\affiliation{\LANL{2}}
\affiliation{\LBNL{2}}
\affiliation{\LehighUniversity{2}}
\affiliation{\LLNL{2}}
\affiliation{\MoreheadState{2}}
\affiliation{\MIT{2}}
\affiliation{\MSU{2}}
\affiliation{\NCKU{2}}
\affiliation{\NCU{2}}
\affiliation{\Nihon{2}}
\affiliation{\NMSU{2}}
\affiliation{\NRNUMEPhI{2}}
\affiliation{\NRCN{2}}
\affiliation{\NTHU{2}}
\affiliation{\NTU{2}}
\affiliation{\ODU{2}}
\affiliation{\Ohio{2}}
\affiliation{\ORNL{2}}
\affiliation{\PNNL{2}}
\affiliation{\Pusan{2}}
\affiliation{\Rice{2}}
\affiliation{\RIKEN{2}}
\affiliation{\Rutgers{2}}
\affiliation{\Saha{2}}
\affiliation{\CFNS{2}}
\affiliation{\StonyBrook{2}}
\affiliation{\RBRC{2}}
\affiliation{\SCNU{2}}
\affiliation{\Seoul{2}}
\affiliation{\Sejong{2}}
\affiliation{\Shinshu{2}}
\affiliation{\Sungkyunkwan{2}}
\affiliation{\TAU{2}}
\affiliation{\Tokyo{2}}
\affiliation{\Tsinghua{2}}
\affiliation{\Tsukuba{2}}
\affiliation{\CUBoulder{2}}
\affiliation{\UCAD{2}}
\affiliation{\UConn{2}}
\affiliation{\UH{2}}
\affiliation{\UIUC{2}}
\affiliation{\UKansas{2}}
\affiliation{\UKY{2}}
\affiliation{\Ljubljana{2}}
\affiliation{\NorthernGeorgia{2}}
\affiliation{\NewHampshire{2}}
\affiliation{\Oslo{2}}
\affiliation{\Regina{2}}
\affiliation{\Seoul{2}}
\affiliation{\USTC{2}}
\affiliation{\UTAustin{2}}
\affiliation{\UTsukuba{2}}
\affiliation{\UTK{2}}
\affiliation{\UTSM{2}}
\affiliation{\UVA{2}}
\affiliation{\Vanderbilt{2}}
\affiliation{\VirginiaTech{2}}
\affiliation{\VirginiaUnion{2}}
\affiliation{\WayneState{2}}
\affiliation{\WI{2}}
\affiliation{\WandM{2}}
\affiliation{\Yamagata{2}}
\affiliation{\Yarmouk{2}}
\affiliation{\Yonsei{2}}
\affiliation{\York{2}}
\affiliation{\Zagreb{2}}

\author{Ralf Seidl}\affiliation{\RIKEN{1}}\affiliation{\RBRC{1}}
\author{Alexey Vladimirov} \affiliation{Universit{\"a}t Regensburg, Regensburg, Germany}
%\author{Daniel Pitonyak}\affiliation{Lebanon Valley College, Annville, PA, USA}
%\author{Alexei Prokudin}\affiliation{Penn State University Berks, Reading, PA, USA}
\author{J.~K.~Adkins}\affiliation{\MoreheadState{1}}
\author{Y.~Akiba}\affiliation{\RIKEN{1}}
\author{A.~Albataineh}\affiliation{\UKansas{1}}
\author{M.~Amaryan}\affiliation{\ODU{1}}
\author{I.~C.~Arsene}\affiliation{\Oslo{1}}
\author{J.~Bae}\affiliation{\Sungkyunkwan{1}}
\author{X.~Bai}\affiliation{\UVA{1}}
\author{M.~Bashkanov}\affiliation{\Yonsei{1}}
\author{R.~Bellwied}\affiliation{\UH{1}}
\author{F.~Benmokhtar}\affiliation{\Duquesne{1}}
\author{J.~C.~Bernauer}\affiliation{\CFNS{1},~\StonyBrook{1},~\RBRC{1}}
\author{F.~Bock}\affiliation{\ORNL{1}}
\author{W.~Boeglin}\affiliation{\FIU{1}}
\author{M.~Borysova}\affiliation{\WI{1}}
\author{E.~Brash}\affiliation{\CNU{1}}
\author{P.~Brindza}\affiliation{\JLab{1}}
\author{W.~J.~Briscoe}\affiliation{\GWU{1}}
\author{M.~Brooks}\affiliation{\LANL{1}}
\author{S.~Bueltmann}\affiliation{\ODU{1}}
\author{M.~H.~S.~Bukhari}\affiliation{\JazanUniversity{1}}
\author{A.~Bylinkin}\affiliation{\UKansas{1}}
\author{R.~Capobianco}\affiliation{\UConn{1}}
\author{W.-C.~Chang}\affiliation{\AcademiaSinica{1}}
\author{Y.~Cheon}\affiliation{\Sejong{1}}
\author{K.~Chen}\affiliation{\CCNU{1}}
\author{K.-F.~Chen}\affiliation{\NTU{1}}
\author{K.-Y.~Cheng}\affiliation{\NCU{1}}
\author{M.~Chiu}\affiliation{\BNL{1}}
\author{T.~Chujo}\affiliation{\UTsukuba{1}}
\author{Z.~Citron}\affiliation{\BGU{1}}
\author{E.~Cline}\affiliation{\CFNS{1},~\StonyBrook{1}}
\author{E.~Cohen}\affiliation{\NRCN{1}}
\author{T.~Cormier}\affiliation{\ORNL{1}}
\author{Y.~Corrales~Morales}
\author{C.~Cotton}\affiliation{\UVA{1}}
\author{C.~Crawford}\affiliation{\UKY{1}}
\author{S.~Creekmore}\affiliation{\ORNL{1}}
\author{C.Cuevas}\affiliation{\JLab{1}}
\author{J.~Cunningham}\affiliation{\ORNL{1}}
\author{G.~David}\affiliation{\BNL{1}}
\author{C.~T.~Dean}\affiliation{\LANL{1}}
\author{M.~Demarteau}\affiliation{\ORNL{1}}
\author{S.~Diehl}\affiliation{\UConn{1}}
\author{N.~Doshita}\affiliation{\Yamagata{1}}
\author{R.~Dupr\'{e}}\affiliation{\IJCLabOrsay{1}}
\author{J.~M.~Durham}\affiliation{\LANL{1}}
\author{R.~Dzhygadlo}\affiliation{\GSI{1}}
\author{R.~Ehlers}\affiliation{\ORNL{1}}
\author{L.~El~Fassi}\affiliation{\MSU{1}}
\author{A.~Emmert}\affiliation{\UVA{1}}
\author{R.~Ent}\affiliation{\JLab{1}}
\author{C.~Fanelli}\affiliation{\MIT{1}}
\author{R.~Fatemi}\affiliation{\UKY{1}}
\author{S.~Fegan}\affiliation{\Yonsei{1}}
\author{M.~Finger}\affiliation{\Charles{1}}
\author{M.~Finger~Jr.}\affiliation{\Charles{1}}
\author{J.~Frantz}\affiliation{\Ohio{1}}
\author{M.~Friedman}\affiliation{\HUJI{1}}
\author{I.~Friscic}\affiliation{\York{1}}
\author{D.~Gangadharan}\affiliation{\UH{1}}
\author{S.~Gardner}\affiliation{\Glasgow{1}}
\author{K.~Gates}\affiliation{\Glasgow{1}}
\author{F.~Geurts}\affiliation{\Rice{1}}
\author{R.~Gilman}\affiliation{\Rutgers{1}}
\author{D.~Glazier}\affiliation{\Glasgow{1}}
\author{E.~Glimos}\affiliation{\ORNL{1}}
\author{Y.~Goto}\affiliation{\RIKEN{1}}
\author{N.~Grau}\affiliation{\AUGIE{1}}
\author{S.~V.~Greene}\affiliation{\Vanderbilt{1}}
\author{A.~Q.~Guo}\affiliation{\IMP{1}}
\author{L.~Guo}\affiliation{\FIU{1}}
\author{S.~K.~Ha}\affiliation{\Yarmouk{1}}
\author{J.~Haggerty}\affiliation{\BNL{1}}
\author{T.~Hayward}\affiliation{\UConn{1}}
\author{X.~He}\affiliation{\GeorgiaState{1}}
\author{O.~Hen}\affiliation{\MIT{1}}
\author{D.~Higinbotham}\affiliation{\JLab{1}}
\author{M.~Hoballah}\affiliation{\IJCLabOrsay{1}}
\author{P.-h.~J.~Hsu}\affiliation{\NTHU{1}}
\author{J.~Huang}\affiliation{\BNL{1}}
\author{G.~Huber}\affiliation{\Regina{1}}
\author{A.~Hutson}\affiliation{\UH{1}}
\author{K.~Y.~Hwang}\affiliation{\Yarmouk{1}}
\author{C.~Hyde}\affiliation{\ODU{1}}
\author{M.~Inaba}\affiliation{\Tsukuba{1}}
\author{T.~Iwata}\affiliation{\Yamagata{1}}
\author{H.-S.~Jo}\affiliation{\Kyungpook{1}}
\author{K.~Joo}\affiliation{\UConn{1}}
\author{N.~Kalantarians}\affiliation{\VirginiaUnion{1}}
\author{K.~Kawade}\affiliation{\Shinshu{1}}
\author{S.~Kay}\affiliation{\Regina{1}}
\author{A.~Kim}\affiliation{\UConn{1}}
\author{B.~Kim}\affiliation{\Sungkyunkwan{1}}
\author{C.~Kim}\affiliation{\Pusan{1}}
\author{M.~Kim}\affiliation{\RIKEN{1}}
\author{Y.~Kim}\affiliation{\Pusan{1}}
\author{Y.~Kim}\affiliation{\Sejong{1}}
\author{E.~Kistenev}\affiliation{\BNL{1}}
\author{V.~Klimenko}\affiliation{\UConn{1}}
\author{S.~H.~Ko}\affiliation{\Seoul{1}}
\author{I.~Korover}\affiliation{\MIT{1}}
\author{W.~Korsch}\affiliation{\UKY{1}}
\author{G.~Krintiras}\affiliation{\UKansas{1}}
\author{S.~Kuhn}\affiliation{\ODU{1}}
\author{C.-M.~Kuo}\affiliation{\NCU{1}}
\author{T.~Kutz}\affiliation{\MIT{1}}
\author{J.~Lajoie}\affiliation{\IowaState{1}}
\author{D.~Lawrence}\affiliation{\JLab{1}}
\author{S.~Lebedev}\affiliation{\IowaState{1}}
\author{J.~S.~H.~Lee}\affiliation{\Seoul{1}}
\author{S.~W.~Lee}\affiliation{\Kyungpook{1}}
\author{Y.-J.~Lee}\affiliation{\MIT{1}}
\author{W.~Li}\affiliation{\Rice{1}}
\author{W.~Li}\affiliation{\CFNS{1},~\StonyBrook{1},~\WandM{1}}
\author{X.~Li}\affiliation{\CIAE{1}}
\author{X.~Li}\affiliation{\LANL{1}}
\author{Y.~T.~Liang}\affiliation{\IMP{1}}
\author{S.~Lim}\affiliation{\Pusan{1}}
\author{C.-h.~Lin}\affiliation{\AcademiaSinica{1}}
\author{D.~X.~Lin}\affiliation{\IMP{1}}
\author{K.~Liu}\affiliation{\LANL{1}}
\author{M.~X.~Liu}\affiliation{\LANL{1}}
\author{K.~Livingston}\affiliation{\Glasgow{1}}
\author{N.~Liyanage}\affiliation{\UVA{1}}
\author{W.~J.~Llope}\affiliation{\WayneState{1}}
\author{C.~Loizides}\affiliation{\ORNL{1}}
\author{E.~Long}\affiliation{\NewHampshire{1}}
\author{R.-S.~Lu}\affiliation{\NTU{1}}
\author{Z.~Lu}\affiliation{\CIAE{1}}
\author{W.~Lynch}\affiliation{\Yonsei{1}}
\author{D.~Marchand}\affiliation{\IJCLabOrsay{1}}
\author{M.~Marcisovsky}\affiliation{\CzechTechUniv{1}}
\author{P.~Markowitz}\affiliation{\FIU{1}}
\author{P.~McGaughey}\affiliation{\LANL{1}}
\author{M.~Mihovilovic}\affiliation{\Ljubljana{1}}
\author{R.~G.~Milner}\affiliation{\MIT{1}}
\author{A.~Milov}\affiliation{\WI{1}}
\author{Y.~Miyachi}\affiliation{\Yamagata{1}}
\author{P.~Monaghan}\affiliation{\CNU{1}}
\author{R.~Montgomery}\affiliation{\Glasgow{1}}
\author{D.~Morrison}\affiliation{\BNL{1}}
\author{C.~Munoz~Camacho}\affiliation{\IJCLabOrsay{1}}
\author{M.~Murray}\affiliation{\UKansas{1}}
\author{K.~Nagai}\affiliation{\LANL{1}}
\author{J.~Nagle}\affiliation{\CUBoulder{1}}
\author{I.~Nakagawa}\affiliation{\RIKEN{1}}
\author{C.~Nattrass}\affiliation{\UTK{1}}
\author{D.~Nguyen}\affiliation{\JLab{1}}
\author{S.~Niccolai}\affiliation{\IJCLabOrsay{1}}
\author{R.~Nouicer}\affiliation{\BNL{1}}
\author{G.~Nukazuka}\affiliation{\RIKEN{1}}
\author{M.~Nycz}\affiliation{\UVA{1}}
\author{V.~A.~Okorokov}\affiliation{\NRNUMEPhI{1}}
\author{S.~Ore$\check{s}$i$\acute{c}$}\affiliation{\Regina{1}}
\author{J.~Osborn}\affiliation{\ORNL{1}}
\author{C.~O'Shaughnessy}\affiliation{\LANL{1}}
\author{S.~Paganis}\affiliation{\NTU{1}}
\author{Z~Papandreou}\affiliation{\Regina{1}}
\author{S.~Pate}\affiliation{\NMSU{1}}
\author{M.~Patel}\affiliation{\IowaState{1}}
\author{C.~Paus}\affiliation{\MIT{1}}
\author{G.~Penman}\affiliation{\Glasgow{1}}
\author{M.~G.~Perdekamp}\affiliation{\UIUC{1}}
\author{D.~V.~Perepelitsa}\affiliation{\CUBoulder{1}}
\author{H.~Periera~da~Costa}\affiliation{\LANL{1}}
\author{K.~Peters}\affiliation{\GSI{1}}
\author{W.~Phelps}\affiliation{\CNU{1}}
\author{E.~Piasetzky}\affiliation{\TAU{1}}
\author{C.~Pinkenburg}\affiliation{\BNL{1}}
\author{I.~Prochazka}\affiliation{\Charles{1}}
\author{T.~Protzman}\affiliation{\LehighUniversity{1}}
\author{M.~Purschke}\affiliation{\BNL{1}}
\author{J.~Putschke}\affiliation{\WayneState{1}}
\author{J.~R.~Pybus}\affiliation{\MIT{1}}
\author{R.~Rajput-Ghoshal}\affiliation{\JLab{1}}
\author{J.~Rasson}\affiliation{\ORNL{1}}
\author{B.~Raue}\affiliation{\FIU{1}}
\author{K.~Read}\affiliation{\ORNL{1}}
\author{K.~R$\o$ed}\affiliation{\Oslo{1}}
\author{R.~Reed}\affiliation{\LehighUniversity{1}}
\author{J.~Reinhold}\affiliation{\FIU{1}}
\author{E.~L.~Renner}\affiliation{\LANL{1}}
\author{J.~Richards}\affiliation{\UConn{1}}
\author{C.~Riedl}\affiliation{\UIUC{1}}
\author{T.~Rinn}\affiliation{\BNL{1}}
\author{J.~Roche}\affiliation{\Ohio{1}}
\author{G.~M.~Roland}\affiliation{\MIT{1}}
\author{G.~Ron}\affiliation{\HUJI{1}}
\author{M.~Rosati}\affiliation{\IowaState{1}}
\author{C.~Royon}\affiliation{\UKansas{1}}
\author{J.~Ryu}\affiliation{\Pusan{1}}
\author{S.~Salur}\affiliation{\Rutgers{1}}
\author{N.~Santiesteban}\affiliation{\MIT{1}}
\author{R.~Santos}\affiliation{\UConn{1}}
\author{M.~Sarsour}\affiliation{\GeorgiaState{1}}
\author{J.~Schambach}\affiliation{\ORNL{1}}
\author{A.~Schmidt}\affiliation{\GWU{1}}
\author{N.~Schmidt}\affiliation{\ORNL{1}}
\author{C.~Schwarz}\affiliation{\GSI{1}}
\author{J.~Schwiening}\affiliation{\GSI{1}}
%\author{R.~Seidl}\affiliation{\RIKEN{1}}
\author{A.~Sickles}\affiliation{\UIUC{1}}
\author{P.~Simmerling}\affiliation{\UConn{1}}
\author{S.~Sirca}\affiliation{\Ljubljana{1}}
\author{D.~Sharma}\affiliation{\GeorgiaState{1}}
\author{Z.~Shi}\affiliation{\LANL{1}}
\author{T.-A.~Shibata}\affiliation{\Nihon{1}}
\author{C.-W.~Shih}\affiliation{\NCU{1}}
\author{S.~Shimizu}\affiliation{\RIKEN{1}}
\author{U.~Shrestha}\affiliation{\UConn{1}}
\author{K.~Slifer}\affiliation{\NewHampshire{1}}
\author{K.~Smith}\affiliation{\LANL{1}}
\author{R.~Soltz}\affiliation{\LLNL{1}}
\author{W.~Sondheim}\affiliation{\LANL{1}}
\author{J.~Song}\affiliation{\CIAE{1}}
\author{J.~Song}\affiliation{\Pusan{1}}
\author{I.~I.~Strakovsky}\affiliation{\GWU{1}}
\author{P.~Steinberg}\affiliation{\BNL{1}}
\author{J.~Stevens}\affiliation{\WandM{1}}
\author{J.~Strube}\affiliation{\PNNL{1}}
\author{P.~Sun}\affiliation{\CIAE{1}}
\author{X.~Sun}\affiliation{\CCNU{1}}
\author{K.~Suresh}\affiliation{\Regina{1}}
\author{W.-C.~Tang}\affiliation{\NCU{1}}
\author{S.~Tapia~Araya}\affiliation{\IowaState{1}}
\author{S.~Tarafdar}\affiliation{\Vanderbilt{1}}
\author{L.~Teodorescu}\affiliation{\BrunelUniversity{1}}
\author{A.~Timmins}\affiliation{\UH{1}}
\author{L.~Tomasek}\affiliation{\CzechTechUniv{1}}
\author{N.~Trotta}\affiliation{\UConn{1}}
\author{T.~S.~Tveter}\affiliation{\Oslo{1}}
\author{E.~Umaka}\affiliation{\IowaState{1}}
\author{A.~Usman}\affiliation{\Regina{1}}
\author{H.~W.~van~Hecke}\affiliation{\LANL{1}}
\author{J.~Velkovska}\affiliation{\Vanderbilt{1}}
\author{E.~Voutier}\affiliation{\IJCLabOrsay{1}}
\author{P.K.~Wang}\affiliation{\IJCLabOrsay{1}}
\author{Q.~Wang}\affiliation{\UKansas{1}}
\author{Y.~Wang}\affiliation{\CCNU{1}}
\author{Y.~Wang}\affiliation{\Tsinghua{1}}
\author{D.~P.~Watts}\affiliation{\Yonsei{1}}
\author{L.~Weinstein}\affiliation{\ODU{1}}
\author{M.~Williams}\affiliation{\MIT{1}}
\author{C.-P.~Wong}\affiliation{\LANL{1}}
\author{L.~Wood}\affiliation{\PNNL{1}}
\author{M.~H.~Wood}\affiliation{\CanisiusCollege{1}}
\author{C.~Woody}\affiliation{\BNL{1}}
\author{B.~Wyslouch}\affiliation{\MIT{1}}
\author{Z.~Xiao}\affiliation{\Tsinghua{1}}
\author{Y.~Yamazaki}\affiliation{\KobeUniversity{1}}
\author{Y.~Yang}\affiliation{\NCKU{1}}
\author{Z.~Ye}\affiliation{\Tsinghua{1}}
\author{H.~D.~Yoo}\affiliation{\Yarmouk{1}}
\author{M.~Yurov}\affiliation{\LANL{1}}
\author{N.~Zachariou}\affiliation{\Yonsei{1}}
\author{W.A.~Zajc}\affiliation{\Columbia{1}}
\author{J.~Zhang}\affiliation{\UVA{1}}
\author{Y.~Zhang}\affiliation{\Tsinghua{1}}
\author{Y.~X.~Zhao}\affiliation{\IMP{1}}
\author{X.~Zheng}\affiliation{\UVA{1}}
\author{P.~Zhuang}\affiliation{\Tsinghua{1}}
%\author{}\affiliation{\NorthernGeorgia{1}}
%\author[\JeonbukNational{1}]{}
%\author[\KoreaUniversity{1}]{}
%\author[\Tokyo{1}]{}
%\author[\UCAD{1}]{}
%\author[\USTC{1}]{}
%\author[\UTAustin{1}]{}
%\author[\UTSM{1}]{}
%\author[\VirginiaTech{1}]{}
%\author[\AANL{1}]{}
%\author[\CUA{1}]{}
%\author[\Duke{1}]{}
%\author[\Hampton{1}]{}
%\author[\HEAROKEK{1}]{}
%\author[\Inha{1}]{}
%\author[\IPAS{1}]{}
%\author[\JAEA{1}]{}
%\author[\JMU{1}]{}
%\author[\LBNL{1}]{}
%\author[\Saha{1}]{}
%\author[\SCNU{1}]{}
%\author[\Zagreb{1}]{}

%\renewcommand\affiliationfont{\itshape\small}

\collaboration{ECCE consortium}  \noaffiliation

==> author_page.tex <==
\makeatletter
\newpage
\centerline
{\large\bf \consortium}
	
\begin{center}
\@author
\end{center}

\makeatother

==> cover_page.tex <==
\renewcommand*\familydefault{\sfdefault}
{\sffamily
\vfill
\vspace{4cm}
\begin{figure}[H]
  \begin{center}
  \includegraphics[width=0.3\linewidth]{figs/ecce-logo.png}
\end{center}
\end{figure}

\makeatletter
\begin{center}
  \large
  {\LARGE{\@title}}

  \begin{tabular}{cc}

%A full-acceptance detector at the EIC based on the BaBAR magnet 
& \today \\
  \end{tabular}
  \end{center}

\vspace{15cm}
\hspace*{0pt}\hfill \notenumber \\
\hspace*{0pt}\hfill \noteversion
\vspace{-15cm}

\vspace{1cm}

\begin{figure}[H]
  \begin{center}
    \includegraphics[width=0.9\linewidth]{figs/ECCE.jpg}
  \end{center}
\end{figure}
}
\makeatother


\vfill
\renewcommand*\familydefault{\rmdefault}

==> exec-summary.tex <==
% A place to put the high level information for the proposal and 
%

\section{Executive Summary}

\paragraph{Name of system / Purpose and scope: \\}
The BABAR/sPHENIX superconducting solenoid provides a central field up to 1.5T, a 2.84m warm bore, and a 3.5m coil length. The stored energy of the magnet is up to 27 MJ, and its operating temperature is 4.5K. This note provides an overview of the BaBar solenoid that will be re-purposed as the ECCE detector solenoid, documents the method by which the in-kind value of the solenoid is estimated. It documents simulations of the magnetic field and the estimated forces on the solenoid coils in the asymmetric ECCE configuration as well as studies of the shape of the magnetic field on the performance of the dual-radiator RICH (dRICH). 

\paragraph{Describe Technology Choice, with reference to Yellow Report: \\}
%The studies in the Yellow Report considered both a low-field (1.4-1.5T) and high field magnet (3.0T). 
The 1.5T magnet discussed here is the BABAR/sPHENIX magnet discussed in section 11.1 of the Yellow Report. Beyond the characteristics already described in the YR this note includes: a decision tree for selection of the the BABAR/sPHENIX magnet, evaluation of forces on the coils, impact of the magnetic field on PID performance in the forward endcap, and in particular on the dRICH performance.
%What is different, same, improved?}

\paragraph{Expected performance of system versus Yellow Report requirements: \\}
The BaBar solenoid provides 
%the 1.4T 
a nominal 1.5 magnetic field to the experiment. The performance of the tracking and momentum resolution 
%in 
including the lower magnetic field is described in the ECCE tracking systems analysis note. 

The field provided by the BaBar solenoid is sufficiently projective that it does not cause a significant smearing of the dRICH ring from the gaseous radiator, and therefore trim coils to shape the magnetic field are not required.  

%Could just be a table.}

\paragraph{Limitations if any for EIC physics: \\}
The nominal 1.5T field of the BaBar magnet taken by itself does not imply any limitations for EIC physics.  The performance of the different detector subsystems (tracking, etc.) are described in additional ECCE working group notes. 
% Include at least one key performance plot and/or links to key performance plots.


==> header.tex <==


\RequirePackage{lineno}
%\input{institute_list}
\usepackage{import}
%\usepackage{titlesec}
\usepackage{enumitem}
\usepackage{amssymb, amsmath}
\usepackage{mathpazo}
\usepackage{float,graphicx}
%\graphicspath{{./}{pCDR/}}
\usepackage[figuresright]{rotating}
\usepackage{wrapfig}
\usepackage[usenames,dvipsnames]{color}
\usepackage{microtype}
\usepackage{tabulary}
%\usepackage{booktabs,multirow,dcolumn,bigdelim}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\usepackage{xr-hyper}
\usepackage[pdftex,plainpages=false,pdfpagelabels,backref,pdfborder={0 0 0}]{hyperref}
%\usepackage{hyperref}
%\usepackage{authblk}
\usepackage{url}
\usepackage[toc,page,titletoc]{appendix}
%\usepackage{afterpage}
\usepackage[font=small,labelfont=bf]{caption}
\setlength\captionmargin{15pt}
\usepackage[scaled]{helvet}
%\usepackage{sectsty}
%\allsectionsfont{\normalfont\sffamily}
%\usepackage{titletoc}
\usepackage{bytefield}
\usepackage{verbatimbox}
\usepackage{tabularx}

%\titlecontents{chapter}
%  [1.5em]
%  {\linespread{0.9}\normalfont\sffamily\bfseries}
%  {\contentslabel{1em}} 
%  {\hspace*{-1.3em}} 
%  {\mdseries\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{section}
%  [3.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{subsection}
%  [4.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\titlecontents{subsubsection}
%  [5.5em]
%  {\linespread{0.9}\normalfont\sffamily}
%  {\contentslabel{2.3em}} 
%  {\hspace*{-2.3em}} 
%  {\titlerule*[1pc]{.}\contentspage} 
%\tolerance = 10000

\usepackage[text={6.5in,8.75in},headheight=26pt,centering]{geometry}
\usepackage{xspace}

\DeclareGraphicsExtensions{.pdf,.png}
\newcommand{\filenamedot}{.}
\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.1in}
\renewcommand{\topfraction} {0.9}
\renewcommand{\bottomfraction} {0.9}
\renewcommand{\textfraction} {0.1}
\renewcommand{\floatpagefraction} {0.8}

%\usepackage{fancyhdr}
%\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
%\renewcommand{\sectionmark}[1]{\markright{#1}{}}
%\fancyhead{} % clear all header fields 
%\fancyhead[RO,LE]{\sffamily \rightmark}
%\fancyhead[LO,RE]{\sffamily \leftmark}
%\fancyfoot{} % clear all footer fields 
%\fancyfoot[RO,LE]{\sffamily \thepage}
%\renewcommand{\headrulewidth}{0pt} 
%\fancypagestyle{plain}{%
%  \fancyhf{}
%  \fancyfoot[RO,LE]{\sffamily \thepage}
%}

\usepackage{multirow}
\usepackage{eurosym}
\usepackage{xcolor}
\usepackage{framed}
\colorlet{shadecolor}{blue!10}

\usepackage{gensymb}

\setcounter{secnumdepth}{3}

\def\consortium{ECCE consortium}
\newcommand{\martinimusic}{\mbox{\sc Martini+Music}\xspace}
\newcommand{\hic}{\mbox{$A$$+$$A$}\xspace}
\newcommand{\pA}{\mbox{$p$$+$$A$}\xspace}
\newcommand{\AuAu}{\mbox{Au$+$Au}\xspace}
\newcommand{\auau}{\mbox{Au$+$Au}\xspace} 
\newcommand{\raa}{\mbox{$R_\mathrm{AA}$}\xspace}
\newcommand{\pbpb}{\mbox{Pb$+$Pb}\xspace} 
\newcommand{\pdau}{\mbox{$p(d)$$+$Au}\xspace} 
\newcommand{\pau}{\mbox{$p$$+$Au}\xspace} 
\newcommand{\aj}{\mbox{$A_J$}\xspace} 
\newcommand {\pp}{\mbox{$p$$+$$p$}\xspace}
\newcommand {\ppbar}{\mbox{$p$$+$$\overline{p}$}\xspace}
\newcommand{\pT}{\mbox{${p_T}$}\xspace}
\newcommand{\jpsi}{\mbox{$J/\psi$}}
\newcommand{\sqrtsnn}{\mbox{$\sqrt{s_{\scriptscriptstyle NN}}$}}
\newcommand{\npart}{$N_\mathrm{part}$}
\newcommand{\ncoll}{$N_\mathrm{coll}$}
\newcommand{\qgp}{\mbox{quark-gluon plasma}\xspace}
\newcommand{\jt}{\mbox{$J_T$}} \newcommand{\qhat}{\mbox{$\hat{q}$}}
\newcommand{\Qsqr}{\mbox{$Q^2$}} \newcommand{\CuCu}{\mbox{Cu$+$Cu}}
\newcommand{\PbPb}{\mbox{Pb$+$Pb}} \newcommand{\pPb}{\mbox{$p$$+$Pb}}
\newcommand{\gjet}{\mbox{$\gamma$-jet}}
\newcommand{\Qmax}{\mbox{$Q_{\max}$}} \newcommand{\ET}{\mbox{$E_T$}}
\newcommand{\Et}{\mbox{$E_T$}} \newcommand{\kt}{\mbox{$k_T$}}
\newcommand{\RAA}{\mbox{$R_{AA}$}\xspace} \newcommand{\IAA}{\mbox{$I_{AA}$}}
\newcommand{\pt}{\mbox{${p_T}$}\xspace}
\newcommand{\highpt}{high-${\rm p_{_{T}}}$}
\newcommand{\lessim}{{\stackrel{<}{\sim}}} \newcommand{\eqnpt}{p_T}
\newcommand{\eA}{\mbox{$e-{\rm A}$}}
\newcommand{\dAu}{\mbox{$d$$+$Au}\xspace}
\newcommand{\pAu}{\mbox{$p$$+$Au}\xspace}
\newcommand{\GeVSQ}{\mbox{${\rm GeV}^2$}}
\newcommand{\fastjet}{\mbox{\sc FastJet}\xspace}
\newcommand{\geant}{\mbox{\sc Geant4}\xspace}
\newcommand{\antikt}{\mbox{anti-$k_T$}\xspace}
\newcommand{\pythia}{\mbox{\sc Pythia}\xspace}
\newcommand{\opera}{\mbox{\sc Opera}\xspace}
\newcommand{\rapgap}{\mbox{\sc Rapgap}\xspace}
\newcommand{\milou}{\mbox{\sc Milou}\xspace}
\newcommand{\pyquen}{\mbox{\sc Pyquen}\xspace}
\newcommand{\hijing}{\mbox{\sc Hijing}\xspace}
\newcommand{\roofit}{\mbox{\sc RooFit}\xspace}
\newcommand{\roounfold}{\mbox{\sc RooUnfold}\xspace}
\newcommand{\beetle}{\mbox{\sc Beetle}\xspace}
\newcommand{\gj}{\mbox{$\gamma$+jet}\xspace}
\newcommand{\gh}{\mbox{$\gamma$+hadron}\xspace}
\newcommand{\martini}{\mbox{\sc Martini}\xspace}
\newcommand{\music}{\mbox{\sc Music}\xspace}

\newcommand{\refdesign}{reference design\xspace}
\newcommand{\refconfig}{reference configuration\xspace}
\newcommand{\dijet}{\mbox{dijet}\xspace}
\newcommand{\fake}{\mbox{fake}\xspace}
\newcommand{\fast}{\mbox{fast}\xspace}
\newcommand{\veryfast}{\mbox{very fast}\xspace}
\newcommand{\epem}{\mbox{$e^+e^-$}\xspace}
\newcommand{\onewidth}{0.6\linewidth}
\newcommand{\twowidth}{0.48\linewidth}
\newcommand{\threewidth}{0.32\linewidth}
\newcommand{\egoing}{\mbox{electron-going}\xspace}
\newcommand{\hgoing}{\mbox{hadron-going}\xspace}
\newcommand{\egodir}{electron-going direction\xspace}
\newcommand{\hgodir}{hadron-going direction\xspace}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}	 
\newcommand{\green}{\color{green}}	 
\newcommand{\magenta}{\color{magenta}}

\newcommand{\lyxdot}{.}
\usepackage{subfig}

\setlength\fboxsep{0pt}
\setlength\fboxrule{0.5pt}
\setlength{\marginparwidth}{2cm}

%\usepackage[textwidth=1in,textsize=footnotesize,disable]{todonotes}
\usepackage[textwidth=1in,textsize=footnotesize]{todonotes}


==> institute_list.tex <==
\newcommand\AANL[1] {\ifnum#1=1 1\else\fi}
\newcommand\AcademiaSinica[1] {\ifnum#1=1 2\else Institute of Physics, Academia Sinica, Taipei, Taiwan\fi}
\newcommand\AUGIE[1] {\ifnum#1=1 3\else Augustana University, Sioux Falls, SD, USA\fi}
\newcommand\BGU[1] {\ifnum#1=1 4\else\fi}
\newcommand\BNL[1] {\ifnum#1=1 5\else Brookhaven National Laboratory, Upton, NY, USA\fi}
\newcommand\BrunelUniversity[1] {\ifnum#1=1 6\else Brunel University London, Uxbridge, UK\fi}
\newcommand\CanisiusCollege[1] {\ifnum#1=1 7\else Canisius College, Buffalo, NY, USA\fi}
\newcommand\CCNU[1] {\ifnum#1=1 8\else Central China Normal University, Wuhan, China\fi}
\newcommand\Charles[1] {\ifnum#1=1 9\else Charles University, Faculty of Maths and Physics, Prague, Czech Republic\fi}
\newcommand\CIAE[1] {\ifnum#1=1 10\else China Institute of Atomic Energy, Fangshan, Beijing, China\fi}
\newcommand\CNU[1] {\ifnum#1=1 11\else Christopher Newport University, Newport News, VA, USA\fi}
\newcommand\Columbia[1] {\ifnum#1=1 12\else Department of Physics, Columbia University, New York, NY, USA\fi}
\newcommand\CUA[1] {\ifnum#1=1 13\else\fi}
\newcommand\CzechTechUniv[1] {\ifnum#1=1 14\else Czech Technical University in Prague, Faculty of Nuclear Sciences and Physical Engineering, Czech Republic\fi}
\newcommand\Duquesne[1] {\ifnum#1=1 15\else Duquesne University, Pittsburgh, PA, USA\fi}
\newcommand\Duke[1] {\ifnum#1=1 16\else\fi}
\newcommand\FIU[1] {\ifnum#1=1 17\else Florida International University, Miami, FL, USA\fi}
\newcommand\GeorgiaState[1] {\ifnum#1=1 18\else Georgia State University, Atlanta, GA, USA\fi}
\newcommand\Glasgow[1] {\ifnum#1=1 19\else School of Physics and Astronomy, University of Glasgow, Glasgow, UK\fi}
\newcommand\GSI[1] {\ifnum#1=1 20\else GSI Helmholtzzentrum fuer Schwerionenforschung, Darmstadt, Germany\fi}
\newcommand\GWU[1] {\ifnum#1=1 21\else The George Washington University, Washington, DC, USA\fi}
\newcommand\Hampton[1] {\ifnum#1=1 22\else\fi}
\newcommand\HEAROKEK[1] {\ifnum#1=1 23\else\fi}
\newcommand\HUJI[1] {\ifnum#1=1 24\else Racah Institute of Physics, Hebrew University, Jerusalem, Israel\fi}
\newcommand\IJCLabOrsay[1] {\ifnum#1=1 25\else Université Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\fi}
\newcommand\IMP[1] {\ifnum#1=1 26\else Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu, China\fi}
\newcommand\Inha[1] {\ifnum#1=1 27\else\fi}
\newcommand\IowaState[1] {\ifnum#1=1 28\else Iowa State University\fi}
\newcommand\IPAS[1] {\ifnum#1=1 29\else\fi}
\newcommand\JAEA[1] {\ifnum#1=1 30\else\fi}
\newcommand\JazanUniversity[1] {\ifnum#1=1 31\else Jazan University, Gizan, Jazan.\fi}
\newcommand\JeonbukNational[1] {\ifnum#1=1 32\else\fi}
\newcommand\JLab[1] {\ifnum#1=1 33\else\fi}
\newcommand\JMU[1] {\ifnum#1=1 34\else\fi}
\newcommand\KobeUniversity[1] {\ifnum#1=1 35\else Graduate School of Science, Kobe University, Kobe, Japan\fi}
\newcommand\KoreaUniversity[1] {\ifnum#1=1 36\else\fi}
\newcommand\Kyungpook[1] {\ifnum#1=1 37\else\fi}
\newcommand\LANL[1] {\ifnum#1=1 38\else Los Alamos National Laboratory, Los Alamos, NM, USA\fi}
\newcommand\LBNL[1] {\ifnum#1=1 39\else\fi}
\newcommand\LehighUniversity[1] {\ifnum#1=1 40\else Lehigh University, Bethlehem, PA, USA\fi}
\newcommand\LLNL[1] {\ifnum#1=1 41\else Lawrence Livermore National Laboratory, Livermore, CA, USA\fi}
\newcommand\MoreheadState[1] {\ifnum#1=1 42\else Morehead State University, Morehad, KY, USA\fi}
\newcommand\MIT[1] {\ifnum#1=1 43\else Massachusetts Institute of Technology, Cambridge, MA, USA\fi}
\newcommand\MSU[1] {\ifnum#1=1 44\else Mississippi State University, Mississippi State, MS, USA\fi}
\newcommand\NCKU[1] {\ifnum#1=1 45\else National Cheng Kung University, Tainan, Taiwan\fi}
\newcommand\NCU[1] {\ifnum#1=1 46\else National Central University, Chungli, Taiwan\fi}
\newcommand\Nihon[1] {\ifnum#1=1 47\else Nihon University, CST, Tokyo, Japan\fi}
\newcommand\NMSU[1] {\ifnum#1=1 48\else New Mexico State University, Las Cruces, NM, USA\fi}
\newcommand\NRNUMEPhI[1] {\ifnum#1=1 49\else National Research Nuclear University MEPhI, Moscow, Russian Federation\fi}
\newcommand\NRCN[1] {\ifnum#1=1 50\else Nuclear Research Center - Negev, Physics Dept., Beer-Sheva, Israel\fi}
\newcommand\NTHU[1] {\ifnum#1=1 51\else National Tsing Hua University, Hsinchu, Taiwan\fi}
\newcommand\NTU[1] {\ifnum#1=1 52\else National Taiwan University, Taipei, Taiwan\fi}
\newcommand\ODU[1] {\ifnum#1=1 53\else Old Dominion University, Department of Physics, Norfolk VA, USA\fi}
\newcommand\Ohio[1] {\ifnum#1=1 53\else Ohio University, Dept. Of Physics and Astronomy, Athens OH, USA\fi}
\newcommand\ORNL[1] {\ifnum#1=1 55\else Oak Ridge National Laboratory, PO Box 2008, Oak Ridge, TN, USA\fi}
\newcommand\PNNL[1] {\ifnum#1=1 56\else Pacific Northwest National Laboratory, Richland, WA, USA\fi}
\newcommand\Pusan[1] {\ifnum#1=1 57\else Pusan National Univeristy, Busan, Republic of Korea\fi}
\newcommand\Rice[1] {\ifnum#1=1 58\else Rice University, Houston, TX, USA\fi}
\newcommand\RIKEN[1] {\ifnum#1=1 59\else RIKEN Nishina Center, Wako, Saitama, Japan\fi}
\newcommand\Rutgers[1] {\ifnum#1=1 60\else The State University of New Jersey, Department of Physics and Astronomy, Piscataway, NJ, USA\fi}
\newcommand\Saha[1] {\ifnum#1=1 61\else\fi}
\newcommand\CFNS[1] {\ifnum#1=1 62\else Center for Frontiers in Nuclear Science, Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA\fi}
\newcommand\StonyBrook[1] {\ifnum#1=1 63\else Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA\fi}
\newcommand\RBRC[1] {\ifnum#1=1 64\else RIKEN BNL Research Center, Brookhaven National Laboratory, Upton, NY, USA\fi}
\newcommand\SCNU[1] {\ifnum#1=1 65\else\fi}
\newcommand\Seoul[1] {\ifnum#1=1 66\else Seoul National University, Seoul, Republic of Korea\fi}
\newcommand\Sejong[1] {\ifnum#1=1 67\else Sejong University, Seoul, Republic of Korea\fi}
\newcommand\Shinshu[1] {\ifnum#1=1 68\else Shinshu University, Matsumoto, Nagano, Japan\fi}
\newcommand\Sungkyunkwan[1] {\ifnum#1=1 69\else Sungkyunkwan University, Suwon, Republic of Korea\fi}
\newcommand\TAU[1] {\ifnum#1=1 70\else\fi}
\newcommand\Tokyo[1] {\ifnum#1=1 71\else\fi}
\newcommand\Tsinghua[1] {\ifnum#1=1 72\else Tsinghua University, Beijing, China\fi}
\newcommand\Tsukuba[1] {\ifnum#1=1 73\else Tsukuba University of Technology, Tsukuba, Ibaraki, Japan.\fi}
\newcommand\CUBoulder[1] {\ifnum#1=1 74\else University of Colorado Boulder, Boulder, CO, USA\fi}
\newcommand\UCAD[1] {\ifnum#1=1 75\else\fi}
\newcommand\UConn[1] {\ifnum#1=1 76\else University of Connecticut, Storrs, CT, USA\fi}
\newcommand\UH[1] {\ifnum#1=1 77\else University of Houston, Houston, TX, USA\fi}
\newcommand\UIUC[1] {\ifnum#1=1 78\else University of Illinois, Urbana, IL, USA\fi}
\newcommand\UKansas[1] {\ifnum#1=1 79\else\fi}
\newcommand\UKY[1] {\ifnum#1=1 80\else\fi}
\newcommand\Ljubljana[1] {\ifnum#1=1 81\else Faculty of Mathematics and Physics, University of Ljubljana, Ljubljana, Slovenia\fi}
\newcommand\NorthernGeorgia[1] {\ifnum#1=1 82\else\fi}
\newcommand\NewHampshire[1] {\ifnum#1=1 83\else University of New Hampshire, Durham, NH, USA\fi}
\newcommand\Oslo[1] {\ifnum#1=1 84\else Department of Physics, University of Oslo, Norway\fi}
\newcommand\Regina[1] {\ifnum#1=1 85\else University of Regina, Regina, SK, Canada\fi}
\newcommand\USeoul[1] {\ifnum#1=1 86\else University of Seoul, Seoul, Republic of Korea\fi}
\newcommand\USTC[1] {\ifnum#1=1 87\else\fi}
\newcommand\UTAustin[1] {\ifnum#1=1 88\fi}
\newcommand\UTsukuba[1] {\ifnum#1=1 89\else University of Tsukuba, Tsukuba, Japan\fi}
\newcommand\UTK[1] {\ifnum#1=1 90\else University of Tennessee, Knoxville, TN, USA\fi}
\newcommand\UTSM[1] {\ifnum#1=1 91\else\fi}
\newcommand\UVA[1] {\ifnum#1=1 92\else University of Virginia, Charlottesville, VA, USA\fi}
\newcommand\Vanderbilt[1] {\ifnum#1=1 93\else Department of Physics and Astronomy, Vanderbilt University, Nashville, TN, USA\fi}
\newcommand\VirginiaTech[1] {\ifnum#1=1 94\else\fi}
\newcommand\VirginiaUnion[1] {\ifnum#1=1 95\else Virginia Union University, Richmond, VA, USA\fi}
\newcommand\WayneState[1] {\ifnum#1=1 96\else Wayne State University, Detroit, MI, USA\fi}
\newcommand\WI[1] {\ifnum#1=1 97\else Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot, Israel\fi}
\newcommand\WandM[1] {\ifnum#1=1 98\else William and Mary, Williamsburg, VA, USA\fi}
\newcommand\Yamagata[1] {\ifnum#1=1 99\else Faculty of Science, Yamagata University, Yamagata, Japan\fi}
\newcommand\Yarmouk[1] {\ifnum#1=1 100\else\fi}
\newcommand\Yonsei[1] {\ifnum#1=1 101\else Yonsei University, Seoul, Republic of Korea\fi}
\newcommand\York[1] {\ifnum#1=1 102\else University of York, York, UK\fi}
\newcommand\Zagreb[1] {\ifnum#1=1 103\else Department of Physics, Faculty of Science, University of Zagreb, Zagreb, Croatia\fi}

==> overview.tex <==
This is the ECCE paper template. The words here are just used for filling space but we will reference plots like Fig.~\ref{fig:BaBarInSPHENIX}, tables such as Tab.~\ref{tab:BaBarStats} and citations~\cite{Lees:2012mma, PDG2020, HFLAV18, Sjostrand:2006za, Sjostrand:2007gs, Agostinelli:2002hh, Allison:2006ve, Lange:2001uf, Golonka:2005pn, Skwarnicki:1986xj, Santos:2013gra, Cowan:2016tnm, AdaBoost, BBDT, Hulsbergen:2005pu, Pivk:2004ty, Wilks:1938dza, Punzi:2003bu}.

\begin{table}[htb]
\footnotesize
\begin{tabularx}{\linewidth}{*{2}{>{\centering\arraybackslash}X}}
\begin{tabular}[b]{|l|l|}
\hline
        Central Induction &  1.5T \\ \hline
        Conductor Peak Field &  2.3T \\ 
        Winding structure &  2 layers \\ 
                          &  graded current density \\ 
        Uniformity in tracking region &  $\pm3\%$ \\ 
        Winding Length &  3512 mm \it{at R.T.} \\ 
        Winding mean radius &  1530 mm \it{at R.T.} \\ 
        Operating Current &  4596 A (4650 A$^{*}$)\\ 
        Inductance &  2.57 H (2.56 H$^{*}$)\\  
        Stored Energy &  27 MJ\\ 
        Total Turns &  1067 \\ 
        Total Length of Conductor &  10,300 m \\ \hline
        $^{*}$ Design Value &   \\ \hline
\end{tabular}
&
\includegraphics[scale=1.3]{figs/BaBar_Shipping.png}     \\
\caption{Main characteristics of the BaBar solenoid, as built.}
\label{tab:BaBarStats}
&
\captionof{figure}{The BaBar solenoid in its shipping cradle.} 
\label{fig:BaBarStats}
\end{tabularx}
\end{table}

\begin{figure}[h!tbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/magnet_install_1.png}
    \caption{The BaBar solenoid in October, 2021, as it was installed in the sPHENIX experiment. The solenoid is resting in the barrel flux return, which will be completed with additional sectors in the coming months.  The experimental cradle, barrel flux return (outer hadronic calorimeter), and BaBar solenoid are all items planned to be re-used by the ECCE experiment.}
    \label{fig:BaBarInSPHENIX}
\end{figure}


% 
% Can be dropped as only one subsection
%
%\subsection{Refurbishment of the BaBar Solenoid}


==> title_page.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\makeatletter
\begin{titlepage}
	
	\vspace*{-1.5cm}
	\noindent
    \begin{flushright}
	    \includegraphics[scale=0.075]{figs/ecce-logo.png} \\
	    \notenumber \\
	    \noteversion \\
	    \today	
    \end{flushright}
	
	\vspace*{2cm}
	
	\begin{center}
		\Large
		\textbf{\@title}
		\normalsize
	\end{center}
	
	\vspace*{0.5cm}
	
	\begin{center}
	    \consortium\footnote{Authors are listed at the end of this paper}
		%\@author
	\end{center}
	
	\vspace*{0.5cm}
	
    \begin{abstract}
        \input{abstract}
    \end{abstract}
	
	\vfill
	
	\begin{flushleft}
% 		BNL/sPHENIX Copyright information...
	\end{flushleft}
	
\end{titlepage}
\makeatother
\renewcommand*{\thefootnote}{\arabic{footnote}}
